Discovery of Endianness and Instruction Size Characteristics in Binary Programs from Unknown Instruction Set Architectures

We study the problem of streamlining reverse engineering (RE) of binary programs from unknown instruction set architectures (ISA). We focus on two fundamental ISA characteristics to beginning the RE process: identification of endianness and whether the instruction width is a fixed or variable. For ISAs with a fixed instruction width, we also present methods for estimating the width. In addition to advancing research in software RE, our work can also be seen as a first step in hardware reverse engineering, because endianness and instruction format describe intrinsic characteristics of the underlying ISA. We detail our efforts at feature engineering and perform experiments using a variety of machine learning models on two datasets of architectures using Leave-One-Group-Out-Cross-Validation to simulate conditions where the tested ISA is unknown during model training. We use bigram-based features for endianness detection and the autocorrelation function, commonly used in signal processing applications, for differentiation between fixed- and variable-width instruction sizes. A collection of classifiers from the machine learning library scikit-learn are used in the experiments to research these features. Initial results are promising, with accuracy of endianness detection at 99.4%, fixed- versus variable-width instruction size at 86.0%, and detection of fixed instruction sizes at 88.0%.

==> Appendices/baselines.tex <==
\subsection{Baselines}\label{appendix:baselines}
\begin{table}[H]
    \centering
    \begin{tabular}{|l||c||c|c|}
        \hline
        \multirow{2}{*}{\textbf{ISA feature}} & \textbf{CpuRec} & \textbf{IsaDetect} & \textbf{IsaDetect} \\
        & \textbf{baseline} & \textbf{baseline - all} & \textbf{baseline - x specified} \\
        \hline
         \textbf{Endianness} & $33/51 = \textbf{0.647}$ & $50287/90465 = \textbf{0.556}$ & $12x/22x = \textbf{0.545}$ \\
        \hline
         \textbf{Fixed/variable} & \multirow{2}{*}{$25/43 = \textbf{0.581}$} & \multirow{2}{*}{$57356/66831 = \textbf{0.858}$} & \multirow{2}{*}{$14x/16x = \textbf{0.875}$} \\ \textbf{instruction size} & & & \\
         \hline
         \textbf{Fixed instruction size} & $17/25 = \textbf{0.680}$ & $52372/57356 = \textbf{0.913}$ & $13x/14x = \textbf{0.929}$ \\
        \hline
    \end{tabular}
\end{table}

==> Appendices/isa_feature_counts.tex <==
\subsection{ISA feature counts}\label{appendix:isa_feature_counts}
\begin{table}[H]
    \centering
    \begin{tabular}{|l||c|c||c|c|}
        \hline
        \multirow{2}{*}{\textbf{ISA feature class}} & \textbf{CpuRec} & \textbf{CpuRec} & \textbf{IsaDetect} & \textbf{IsaDetect} \\
        & \textbf{class count} & \textbf{file count} & \textbf{class count} & \textbf{file count} \\
        \hline
         \textbf{Little endian} & 33 & 33 & 12 & 50287 \\
        \hline
         \textbf{Big endian} & 18 & 18 & 10 & 40178 \\
        \hline
         \textbf{Endianness total} & 51 & 51 & 22 & 90465 \\
        \hline
         \textbf{Instruction size 16} & 6 & 6 & 0 & 0 \\
         \hline
         \textbf{Instruction size 24} & 1 & 1 & 0 & 0 \\
         \hline
         \textbf{Instruction size 32} & 17 & 17 & 13 & 52372 \\
         \hline
         \textbf{Instruction size 128} & 1 & 1 & 1 & 4984 \\
        \hline
         \textbf{Fixed instruction size} & 25 & 25 & 14 & 57356 \\
        \hline
         \textbf{Variable instruction size} & 18 & 18 & 2 & 9475 \\
         \hline
         \textbf{Fixed/variable} & \multirow{2}{*}{43} & \multirow{2}{*}{43} & \multirow{2}{*}{16} & \multirow{2}{*}{66831} \\ \textbf{instruction size total} & & & & \\
        \hline
    \end{tabular}
\end{table}

==> Appendices/isadetect_filecounts.tex <==
\subsection{IsaDetect file counts}\label{appendix:isadetect_filecounts}
\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|}
\hline
\textbf{ISA}  & \textbf{File count}\\\hline
alpha         & 3971\\\hline
amd64         & 4366\\\hline
arm64         & 3636\\\hline
armel         & 4000\\\hline
armhf         & 3995\\\hline
hppa          & 4830\\\hline
i386          & 5109\\\hline
ia64          & 4984\\\hline
m68k          & 4400\\\hline
mips          & 3565\\\hline
mips64el      & 4312\\\hline
mipsel        & 3775\\\hline
powerpc       & 3631\\\hline
powerpcspe    & 3961\\\hline
ppc64         & 2833\\\hline
ppc64el       & 3523\\\hline
riscv64       & 4440\\\hline
s390          & 5164\\\hline
s390x         & 3538\\\hline
sh4           & 5930\\\hline
sparc         & 4980\\\hline
sparc64       & 3276\\\hline
x32           & 4176\\\hline
\hline
\textit{Total} & 96395\\\hline 
    \end{tabular}
    % \caption{Table of number of files for each ISA in the ISADetect datasets.}
\end{table}


==> Appendices/labels.tex <==
\subsection{Labels}\label{appendix:labels}
\begin{longtable}{|l|l|l|l|l|}
    \hline
        \textbf{IsaDetect} & \textbf{CpuRec} & \textbf{Wordsize} & \textbf{Endianness} & \textbf{Instruction Size} \\ \hline
~          & 6502.corpus        & 8        & LE & 8-32 \\ \hline  
~          & 68hc08.corpus      & 8        & BE & 8-16 \\ \hline  
~          & 68hc11.corpus      & 8        & BE & 8-40 \\ \hline  
~          & 8051.corpus        & 32       & LE & 8-128 \\ \hline 
arm64      & arm64.corpus       & 64       & LE & 32 \\ \hline    
~          & armeb.corpus       & 32       & BE & 32 \\ \hline    
armel      & armel.corpus       & 32       & LE & 32 \\ \hline    
armhf      & armhf.corpus       & 32       & LE & 32 \\ \hline    
~          & arcompact.corpus   & 32       & LE & 16-32 \\ \hline 
~          & avr.corpus         & 8        & LE & 16-32 \\ \hline 
alpha      & alpha.corpus       & 64       & LE & 32 \\ \hline    
~          & axiscris.corpus    & 32       & LE & 16 \\ \hline    
~          & blackfin.corpus    & 32       & LE & 16-32 \\ \hline 
~          & clipper.corpus     & 32       & LE & 2-8 \\ \hline   
~          & cuda.corpus        & 32       & LE & 32 \\ \hline    
~          & cell-spu.corpus    & 32       & BE & 32 \\ \hline    
~          & compactrisc.corpus & 16       & LE & 16 \\ \hline    
~          & cray.corpus        & 64       & NA & ~ \\ \hline     
~          & epiphany.corpus    & 32       & LE & 16-32 \\ \hline 
~          & fr-v.corpus        & 32       & NA & ~ \\ \hline     
~          & fr30.corpus        & 32       & BE & 16 \\ \hline    
~          & ft32.corpus        & 32       & NA & ~ \\ \hline     
~          & h8-300.corpus      & 8        & BE & 8-16 \\ \hline  
~          & h8s.corpus         & 16       & BE & ~ \\ \hline     
~          & hp-focus.corpus    & 32       & NA & ~ \\ \hline     
hppa       & hp-pa.corpus       & 64       & BE & 32 \\ \hline    
~          & ia-64.corpus       & 64       & LE & 128 \\ \hline   
~          & iq2000.corpus      & 32       & BE & ~ \\ \hline     
~          & m32c.corpus        & 32       & NA & ~ \\ \hline     
~          & m32r.corpus        & 32       & BI & 16-32 \\ \hline 
m68k       & m68k.corpus        & 32       & BE & ~ \\ \hline     
~          & m88k.corpus        & 32       & BI & 32 \\ \hline    
~          & mcore.corpus       & 32       & BE & 16 \\ \hline    
mips64el   & ~                  & 64       & LE & 32 \\ \hline    
~          & mips16.corpus      & 16       & BI & 16 \\ \hline    
mips       & mipseb.corpus      & 32       & BE & 32 \\ \hline    
mipsel     & mipsel.corpus      & 32       & LE & 32 \\ \hline    
~          & mmix.corpus        & 64       & BE & 32 \\ \hline    
~          & mn10300.corpus     & 32       & LE & ~ \\ \hline     
~          & msp430.corpus      & 16       & LE & ~ \\ \hline     
~          & mico32.corpus      & 32       & BE & 32 \\ \hline    
~          & microblaze.corpus  & 32/64    & BI & 32 \\ \hline    
~          & moxie.corpus       & 32       & BI & 32-48 \\ \hline 
~          & nds32.corpus       & 32/16    & BI & 16-32 \\ \hline 
~          & nios-ii.corpus     & 32       & LE & 32 \\ \hline    
~          & ocaml.corpus       & NA       & NA & ~ \\ \hline     
~          & pdp-11.corpus      & 16       & LE & 16 \\ \hline    
~          & pic10.corpus       & 8        & LE & ~ \\ \hline     
~          & pic16.corpus       & 8        & LE & ~ \\ \hline     
~          & pic18.corpus       & 8        & LE & ~ \\ \hline     
~          & pic24.corpus       & 16       & LE & 24 \\ \hline    
ppc64      & ppceb.corpus       & 64       & BE & ~ \\ \hline     
ppc64el    & ppcel.corpus       & 64       & LE & ~ \\ \hline     
riscv64    & risc-v.corpus      & 64       & LE & 32 \\ \hline    
~          & rl78.corpus        & 16       & LE & ~ \\ \hline     
~          & romp.corpus        & 32       & BE & 8-32 \\ \hline  
~          & rx.corpus          & 16/32/64 & LE & ~ \\ \hline     
s390x      & ~                  & 64       & BE & ~ \\ \hline     
s390       & s-390.corpus       & 32       & BE & ~ \\ \hline     
sparc      & ~                  & 32       & BE & 32 \\ \hline    
sparc64    & sparc.corpus       & 64       & BE & 32 \\ \hline    
~          & stm8.corpus        & 8        & ~  & ~ \\ \hline     
~          & stormy16.corpus    & 16       & LE & ~ \\ \hline     
sh4        & superh.corpus      & 32       & BI & ~ \\ \hline     
~          & tilepro.corpus     & 32       & ~  & ~ \\ \hline     
~          & tlcs-90.corpus     & 8        & ~  & ~ \\ \hline     
~          & tms320c2x.corpus   & 16/32    & ~  & ~ \\ \hline     
~          & tms320c6x.corpus   & 32       & BI & ~ \\ \hline     
~          & trimedia.corpus    & ~        & ~  & ~ \\ \hline     
~          & v850.corpus        & 32       & ~  & ~ \\ \hline     
~          & visium.corpus      & 32       & ~  & ~ \\ \hline     
~          & wasm.corpus        & 32       & LE & ~ \\ \hline     
~          & we32000.corpus     & 32       & ~  & ~ \\ \hline     
amd64      & x86-64.corpus      & 64       & LE & 8-120 \\ \hline 
i386       & x86.corpus         & 32       & LE & 8-120 \\ \hline 
~          & xtensa.corpus      & 32       & BI & 16-24 \\ \hline 
~          & z80.corpus         & 8        & LE & 8-32 \\ \hline  
~          & i860.corpus        & 32/64    & BI & ~ \\ \hline     
ia64       & ~                  & 64       & LE & 128 \\ \hline   
x32        & ~                  & 32       & LE & ~ \\ \hline     
powerpc    & ~                  & 32       & BE & 32 \\ \hline    
powerpcspe & ~                  & 32       & BE & 32 \\ \hline    
~          & 78k.corpus         & 8 or 16  & ~  & ~ \\ \hline    
\end{longtable}

==> Appendices/parameter_tuning.tex <==
\subsection{Parameter tuning}\label{appendix:parameter_tuning}

\newcommand{\hyperparmcaptionnodot}[5]{Comparison of \MakeLowercase{{#1}} for the {#4} feature. Detection of {#2}. Trained and tested on {#3}, with {#5} files per ISA}
\newcommand{\hyperparmcaption}[5]{\hyperparmcaptionnodot{#1}{#2}{#3}{#4}{#5}.}
\newcommand{\hyperparmcaptionvar}[9]{\hyperparmcaptionnodot{#1}{#2}{#3}{#4}{#5}, with powers of {#6} of the \texttt{\MakeLowercase{{#7}}} parameter from {#8} to {#9}.}

\newcommand{\hyperparmcaptionentirenodot}[4]{Comparison of \MakeLowercase{{#1}} for the {#4} feature. Detection of {#2}. Trained and tested on the entire {#3} dataset}
\newcommand{\hyperparmcaptionentire}[4]{\hyperparmcaptionentirenodot{#1}{#2}{#3}{#4}.}
\newcommand{\hyperparmcaptionentirevarnodot}[8]{\hyperparmcaptionentirenodot{#1}{#2}{#3}{#4} with powers of {#5} of the \texttt{\MakeLowercase{{#6}}} parameter from {#7} to {#8}}
\newcommand{\hyperparmcaptionentirevar}[8]{\hyperparmcaptionentirevarnodot{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}.}






\subsubsection{Feature parameter tuning}\label{appendix:feature_parameter_tuning}
\paragraph{Fixed/Variable instruction size - AutoCorrelation}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/autocorr_tuning/isvar_AutoCorrelation.png}
    \caption{\hyperparmcaptionentirevar{\texttt{Lag}}{fixed/variable instruction size}{CpuRec}{AutoCorrelation}{two}{\texttt{Lag}}{16}{1024}}
    \label{fig:featureparam Fixed/Variable instruction size - AutoCorrelation}
\end{figure}

\paragraph{Fixed/Variable instruction size - Fourier}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/fourier_tuning/isvar_None_Fourier.png}
    \caption{\hyperparmcaptionentirevar{\texttt{data\_half\_len}}{fixed/variable instruction size}{CpuRec}{Fourier}{two}{\texttt{data\_half\_len}}{16}{1024} Note that \texttt{data\_half\_len} for the SVC classifier are no lower than 32, as lower frequencies drastically increase training time.}
    \label{fig:featureparam Fixed/Variable instruction size - Fourier}
\end{figure}

\paragraph{Fixed instruction size - AutoCorrelation}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/autocorr_tuning/instsize_AutoCorrelation.png}
    \caption{\hyperparmcaptionentirevar{\texttt{Lag}}{fixed instruction size}{CpuRec}{AutoCorrelation}{two}{\texttt{Lag}}{16}{512}}
    \label{fig:featureparam Fixed instruction size - AutoCorrelation}
\end{figure}

\paragraph{Fixed instruction size - Fourier}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/fourier_tuning/instsize_None_Fourier.png}
    \caption{\hyperparmcaptionentirevar{\texttt{data\_half\_len}}{fixed instruction size}{CpuRec}{Fourier}{two}{\texttt{data\_half\_len}}{16}{1024}}
    \label{fig:featureparam Fixed instruction size - Fourier}
\end{figure}






\subsubsection{Classifier hyperparameter tuning}\label{appendix:hyperparameter_tuning}
\paragraph{Endianness - 100 files per architecture}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/endianness_full_100_EndiannessSignatures.png}
    \caption{\hyperparmcaptionvar{Hyperparameters}{endianness detection}{IsaDetectFull}{endianness signatures}{100}{ten}{c}{$10^{1}$}{$10^{11}$}}
    \label{fig:hyperparam Endianness, endianness signatures, full - 100}
\end{figure}



\paragraph{Endianness}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/endianness_full_30_EndiannessSignatures.png}
    \caption{\hyperparmcaptionvar{Hyperparameters}{endianness detection}{IsaDetectFull}{endianness signatures}{30}{ten}{c}{$10^{1}$}{$10^{11}$}}
    \label{fig:hyperparam Endianness, endianness signatures, full}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/endianness_full_30_Bigrams.png}
    \caption{\hyperparmcaptionvar{Hyperparameters}{endianness detection}{IsaDetectFull}{bigrams}{30}{ten}{c}{$10^{1}$}{$10^{10}$}}
    \label{fig:hyperparam Endianness, bigrams, full}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/endianness_code_30_EndiannessSignatures.png}
    \caption{\hyperparmcaptionvar{Hyperparameters}{endianness detection}{IsaDetectCode}{endianness signatures}{30}{ten}{c}{$10^{1}$}{$10^{11}$}}
    \label{fig:hyperparam Endianness, endianness signatures, code}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/endianness_code_30_Bigrams.png}
    \caption{\hyperparmcaptionvar{Hyperparameters}{endianness detection}{IsaDetectCode}{bigrams}{30}{ten}{c}{$10^{1}$}{$10^{10}$}}
    \label{fig:hyperparam Endianness, bigrams, code}
\end{figure}



\paragraph{Fixed/variable instruction size}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/isvar_None_ByteDifferencePrimes.png}
    \caption{\hyperparmcaptionentirevar{Hyperparameters}{fixed/variable instruction size}{CpuRec}{ByteDifferencePrimes}{ten}{\texttt{c}}{$10^{-4}$}{$10^6$}}
    \label{fig:hyperparam isvar, ByteDifferencePrimes}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/isvar_None_AutoCorrelation_1-32.png}
    \caption{\hyperparmcaptionentirevar{Hyperparameters}{fixed/variable instruction size}{CpuRec}{AutoCorrelation}{ten}{\texttt{c}}{$10^{-1}$}{$10^6$}}
    \label{fig:hyperparam isvar, AutoCorrelation}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/isvar_None_Fourier.png}
    \caption{\hyperparmcaptionentirevar{Hyperparameters}{fixed/variable instruction size}{CpuRec}{Fourier}{ten}{\texttt{c}}{$10^{-7}$}{$10^9$}}
    \label{fig:hyperparam isvar, Fourier}
\end{figure}



\paragraph{Fixed instruction size}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/instsize_None_AutoCorrelation.png}
    \caption{\hyperparmcaptionentirevar{Hyperparameters}{fixed instruction size}{CpuRec}{AutoCorrelation}{ten}{\texttt{c}}{$10^{-7}$}{$10^7$}}
    \label{fig:hyperparam instsize, AutoCorrelation}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/instsize_None_Fourier.png}
    \caption{\hyperparmcaptionentirevar{Hyperparameters}{fixed instruction size}{CpuRec}{Fourier}{ten}{\texttt{c}}{$10^{-7}$}{$10^9$}}
    \label{fig:hyperparam instsize, Fourier}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/40_Results/hyperparameter_tuning/instsize_None_AutoCorrelationPeak3_1-32.png}
    \caption{\hyperparmcaptionentirevar{Hyperparameters}{fixed instruction size}{CpuRec}{Fourier}{ten}{\texttt{c}}{$10^{-7}$}{$10^7$}}
    \label{fig:hyperparam instsize, AutoCorrelationPeak3}
\end{figure}


